Learning Controllable Fair Representations

Learning data representations that are transferable and are fair with respect to certain protected attributes is crucial to reducing unfair decisions while preserving the utility of the data. We propose an information-theoretically motivated objective for learning maximally expressive representations subject to fairness constraints. We demonstrate that a range of existing approaches optimize approximations to the Lagrangian dual of our objective. In contrast to these existing approaches, our objective allows the user to control the fairness of the representations by specifying limits on unfairness. Exploiting duality, we introduce a method that optimizes the model parameters as well as the expressiveness-fairness trade-off. Empirical evidence suggests that our proposed method can balance the trade-off between multiple notions of fairness and achieves higher expressiveness at a lower computational cost.

==> 2_mi.tex <==
 \section{AN INFORMATION-THEORETIC OBJECTIVE FOR CONTROLLABLE FAIR REPRESENTATIONS}
 \label{sec:mi}

\subsection{Desiderata}
We consider the case in which we are given a dataset $\mc{D}_u = \{\xui\}_{i=1}^{M}$ containing pairs of observations $\xv \in \mc{X}$ and sensitive attributes $\uv \in \mc{U}$. We assume the dataset is sampled i.i.d. from an unknown data distribution $\qxu$. 
%Let $\qzixu$ denote an encoder distribution (parameterized by $\phi \in \Phi$) that is used to create the representation $\zv$.
We wish to find a mechanism to transform each data point $(\xv, \uv)$ into a new \emph{representation} $\zv \in \mc{Z}$ that 
is (1) \emph{transferable}, meaning that it can be used in place of $(\xv, \uv)$ by multiple unknown vendors on a variety of downstream tasks, and (2) \emph{fair}, meaning that the sensitive attributes $\uv$ are protected.
%\textit{fair and transferable}, and can be used by multiple unknown vendors and protects sensitive attributes. 
%\se{i would define formally what a representation is. people will wonder if it is a (stochastic) function of x and/or u. and why learn?}\js{replace learn with find, here I define representations are samples from RV instead of the function, they have to be vectors otherwise you cannot classify over them i think.}
% \s{we need to say $z$ is a random variable if you want to use mutual information}
For conciseness, we focus on the \textit{demographic parity} notion of fairness \citep{calders2009building,zliobaite2015on,zafar2015learning}, which requires the decisions made by a classifier over $\zv$ to be independent of the sensitive attributes $\uv$. We discuss in Appendix~\ref{app:eodds-eopp} how our approach can be extended to control other notions of fairness simultaneously, such as the \textit{equalized odds} and \textit{equalized opportunity} notions of fairness~\citep{hardt2016equality}.

We assume the representations $\zv \in \mc{Z}$ for $(\xv, \uv)$ are obtained by sampling from a conditional probability distribution $\qzixu$ parameterized by $\phi \in \Phi$. The joint distribution of $(\xv, \zv, \uv)$ is then $\qxzu = \qxu \qzixu$.
We formally express our desiderata for $\zv$ through the concept of mutual information:
%concerning the random variables $\Zv, \Xv, \Uv$ and the distribution $Q$:
%
%\s{before using MI, i think we need to specify a probability space. probably up where you define the dataset}\js{okay but maybe we want to keep most of the existing notation intact}
\begin{enumerate}
\item{\textbf{Fairness}} \\\x{The representation} $\zv$ should have low mutual information with the sensitive attributes $\uv$.
\item{\textbf{Expressiveness}} \\\x{The representation} $\zv$ should have high mutual information with the observations $\xv$ conditioned on $\uv$ \rk{Is this necessary:}(in expectation over possible values of $\uv$).
%\s{not quite rigorous, you might need to say in expectation over possible values of u} \js{added}
\end{enumerate}
The first condition encourages $\zv$ to be independent of $\uv$; if this is the case, the downstream vendor cannot learn a classifier over the representations $\zv$ that discriminates based on $\uv$. Intuitively, the mutual information $\iq(\zv, \uv)$ is related to the optimal predictor of $\uv$ given $\zv$. If $\iq(\zv, \uv)$ is zero, then no classifier could perform better than random chance; if $\iq(\zv, \uv)$ is large, vendors in downstream tasks could utilize $\zv$ to predict the sensitive attributes $\uv$  and make unfair decisions.

The second condition encourages $\zv$ to contain as much information as possible from $\xv$ conditioned on the knowledge of $\uv$; by conditioning on $\uv$, we ensure we do not encourage information in $\xv$ that is correlated with $\uv$ to leak into $\zv$. In general, the two desiderata allow $\zv$ to encode non-sensitive information from $\xv$ (expressiveness) while excluding information in $\uv$ (fairness).

% \js{cite relevant paper in ICML}

% this does not encourage information of $\uv$ to leak into $\zv$ since $\uv$ is already known. 

% Let $\qxu$ denote the data distribution of $\mc{D}_u$ and let $\qzixu$ denote an encoder distribution (parameterized by $\phi \in \Phi$) that is used to create the representation $\zv$; then the joint distribution of $(\xv, \zv, \uv)$ is $\qxzu = \qxu \qzixu$.
% \s{move this part up}

\tmp{\s{does it ever make sense to have stochastic mapping to features?}}

Our goal is to choose parameters $\phi \in \Phi$ for $\qzixu$ such that both criteria are met\footnote{Note that is not sufficient to simply ignore $\uv$ as an input, as $\xv$ may still contain information about $\uv$.}. Because we wish to ensure our representations satisfy fairness constraints even when at the cost of using less expressive $\zv$, we synthesize the two desiderata into the following constrained optimization problem:
\begin{gather} 
\max_{\phi \in \Phi} \iq(\xv; \zv | \uv) \qquad \qquad \text{s.t. } \iq(\zv; \uv) < \epsilon \label{eq:constraint-objective}
\end{gather}
%\s{incorrect, missing an expectation over u}\js{actually I think this notation implicitly consideres expectation over u, also the definition of conditional mutual information also contains the expectation over $u$. See \url{https://en.wikipedia.org/wiki/Conditional_mutual_information}}
where $\iq(\xv; \zv | \uv)$ denotes the mutual information of $\xv$ and $\zv$ conditioned on $\uv$,
%over $q(\uv)$
$\iq(\zv; \uv)$ denotes mutual information between $\zv$ and $\uv$, and the hyperparameter $\epsilon > 0$ controls the maximum amount of mutual information allowed between $\zv$ and $\uv$. The motivation of our ``hard'' constraint on $I_q(\zv; \uv)$ -- as opposed to a ``soft'' regularization term -- is that even at the cost of learning less expressive $\zv$ and losing some predictive power, we view as important ensuring that our representations are fair to the extent dictated by $\epsilon$. 

\begin{comment}
Note that $\epsilon>0$ allows a slight violation of exact demographic parity (where $\iq(\zv, \uv) = 0$) %\s{exact fairness never defined} 
such that the parameter space $\Phi$ contains at least one feasible solution, accounting for the fact that our encoder $\qzixu$ has limited capacity.\footnote{Note that is not sufficient to simply ignore $\uv$ as an input, as $\xv$ may still contain information about $\uv$.} Having a positive $\epsilon$ also allows us to consider multiple notions of fairness in fair representation learning; since different notions of fairness could be incompatible, we would like to find a reasonable trade-off between one another. 
\end{comment}
%and we are willing to sacrifice a reasonable amount of ``demographic parity'' fairness to achieve higher performance on the other task. 
%\s{last two sentences not super clear}\js{did a fix}



% \s{might add some discussion of how to translate $\epsilon$ to ``accuracy in predicting u from z''. if MI is zero, then no classifier can do better than random chance. etc.}\js{fixed}

Both mutual information terms in Equation~\ref{eq:constraint-objective} are difficult to compute and optimize. In particular, the optimization objective $\iq(\xv; \zv|\uv)$  in Equation~\ref{eq:constraint-objective} is the following expectation:
\begin{align*}
&\iq(\xv; \zv | \uv) \\
= & \ \bb{E}_{\qxzu}[\log \qxziu - \log \qxiu - \log \qziu]    
\end{align*}
while the constraint on $\iq(\zv; \uv)$ involves the following expectation:
\begin{align*}
\iq(\xv; \zv | \uv) =  \ \bb{E}_{\qzu}[\log \qziu - \log \qz]    
\end{align*}
%where 
%\begin{gather*}
%\qziu = \sum_{\xv} \qzixu \qx \\
%\qxziu = \frac{\qxzu}{\sum_{\xv, \zv}\qxzu}
%\end{gather*}
Even though $\qzixu$ is known analytically (and assumed to be easy to evaluate), both mutual information terms are difficult to estimate and evaluate. This is because of the term $\log \qziu = \log \sum_{\xv} \qzixu \qx$ in both $\iq(\xv; \zv | \uv)$ and $\iq(\xv; \zv | \uv)$ %is not immediately tractable from a tractable $\qzixu$ %requires integration over $q(\xv)$, 
requires us to compute the sum over the entire training dataset, which is unfeasible for stochastic gradient descent training.
\s{seems wrong}
%\s{if we have a one sentence argument for why, add. or maybe add a citation}

\subsection{Tractable Bounds for Mutual Information Objectives}


\begin{comment}
whose gradient over $\phi$ relies on $\log (\qxziu / \qziu)$, where 
\begin{gather*}
\qxziu = \qxzu / \qu \\
\qziu = \qzu / \qu \\
\end{gather*}
and $
\qzu = \sum_x \qzixu \qxu
$
is the marginal distribution over $(\zv, \uv)$, and $\qu = \sum_{\xv \in \mc{X}} \qxu$ is the marginal distribution over $\uv$. 
%  \s{empirical distributions never defined..keep terminology consistent with what you defined earlier}
% \rk{Why is q(u) said to be an (unparameterized) empirical distribution in the last sentence? (And it's used later in the paper too)}
It is not possible to write the gradient of $\iq(\xv; \zv | \uv)$ as a tractable expression in terms of $\log \qzixu$, 
\s{seems reasonable, but do we have a proof? it's always hard to prove something is not possible..}\js{i guess we can try to write more on this if we have more time? I guess this is slightly lower priority than other issues.}
which is tractable; a similar derivation holds for $\iq(\zv; \uv)$.
\end{comment}
% \done{\rk{Someone double check my rewrite of this last sentence is mathematically correct.}\js{the issues is what we define as ``tractable'', maybe stefano can take a look?}}

Our strategy will be to obtain upper and lower bounds to these mutual information terms, which do have tractable gradient estimates; we introduce the following lemmas, with the proofs provided in Appendix~\ref{sec:proofs}. We note that similar bounds have been proposed in \citep{alemi2016deep,alemi2017fixing,zhao2018a}. %\s{fix citation}

% \done{\js{we should not put the proofs here, but we need to mention the gap between the tractable thing and the intractable thing, so i wonder if we should state the lemma with equalities, and then the bounds are straightforward} \rk{<-- Don't understand this comment, sorry!}}

% \rk{Do we not need to citep Alemi (or anyone) for the bounds?} \js{sure we should citep then and ourselves}

We begin with a (variational) \emph{lower} bound on the objective  function $\iq(\xv; \zv | \uv)$ we would like to \emph{maximize} in Equation~\ref{eq:constraint-objective} 
\begin{lemma} \label{thm:reconstruction}
For any conditional distribution $p(\xv|\zv, \uv)$
\begin{align}
\label{eq:mi:lb}
\iq(\xv; \zv | \uv) &= \underbrace{\bb{E}_{\qxzu}[\log p_\theta(\xv|\zv, \uv)] + \hq(\xv | \uv)}_{\mc{L}_r: \text{Lower bound to } \iq(\xv; \zv | \uv)} \\
\nonumber
&+ \bb{E}_{\qzu}\KL(\qxizu \Vert p_\theta(\xv|\zv, \uv))
\end{align}
where $\hq(\xv|\uv)$ is the entropy of $\xv$ conditioned on $\uv$, and $\KL$ denotes KL-divergence.
\end{lemma}

Next, we provide an \emph{upper} bound for the term in the constraint $\iq(\zv; \uv)$ (which we implicitly want to \emph{minimize}):
\begin{lemma} \label{thm:elbo}
For any distribution $\pz$
\begin{align}
 & \iq(\zv; \uv) \leq \iq(\xv; \zv|\uv) \label{eq:mi:2} \  \\
= & \ \underbrace{\bb{E}_{\qxu}\KL(\qzixu \Vert \pz)}_{C_1: \text{Loose upper bound to }\iq(\zv; \uv)} - \KL(\qz \Vert \pz) \nonumber
\end{align}
\end{lemma}

% \done{\rk{In the 2nd and 3rd line of the above proof, shouldn't it be $\log\qzixu$ instead of $\log\qxuiz$?}\js{fixed}}

% \s{i would swap in the bounds with slack terms like in appendix}
% \s{need to tell the reader why we came up with two bounds..}

% \s{there should be paragraph here elaborating on tractability of these bounds. choose p from family with tractable ..}

% \s{then, tightness}

%In these lemmas we obtained a lower bound for $I_q(\xv; \zv | \uv)$ (which we wish to maximize) and an upper bound for $I_q(\zv; \uv)$ (which we wish to minimize). 
Crucially, if we $p(\xv|\zv, \uv)$ and $\pz$ are distributions with tractable log probabilities (such as Bernoulli / Gaussian), \s{evaluations? why estimates? sampling? be precise}, 
then these bounds can be tractably estimated and have tractable Monte Carlo gradient estimates (as $\qzixu$ is assumed to be tractable).

\s{we denote this bound $C_1$}

\subsection{Tightening Bounds with Variational Autoencoders}

The quality (tightness) of these bounds depends on the choices of $p_\theta(\xv|\zv, \uv)$ and $\pz$.
In order to encourage these bounds to be tight (with respect to the true mutual information), 
%we consider choosing $p(\xv|\zv, \uv)$ and $\pz$ from the family of distributions with tractable density estimates, and 
we find $\pxizu$ and $\pz$ that are close to $\qxizu$, $\qz$ (for which we lack tractable density estimates), respectively.
% \a{$\pxizu$ and $p(\xv|\zv, \uv)$ are used interchangeably everywhere but one contains $\theta$, other doesn't} 
For example, it is clear from Equation~\ref{eq:mi:lb} that $p(\xv|\zv, \uv)$ should be close to $\qxizu$ to eliminate the slack term. A similar argument goes for $\pz$ and $\qz$ in Equation~\ref{eq:mi:2}, where we would like $\KL(\qz \Vert \pz)$ to be small for the bound to be tight. 
% \s{need similar justification for the other pieces, why we want them to be similar to q} Next, we elaborate on how to choose $p(\xv|\zv, \uv)$, $\pz$ and $\pu$. 

\s{agreed with aditya. need to stick with one notation, with or without theta. this is confusing}\js{added theta to $\pxizu$}

%\s{sloppy. not really true. can only estimate from data}
% \s{why is this a good idea? convince people}
% \rk{Confirm this is still right}
% \done{\rk{Why don't we choose p(u) to be q(u) exactly and just change lemma 3 to prove a lower bound? Is it just so we can claim we're using an upper bound? Do we get any actual (empirical?) benefit out of this choice?} \js{because we need to evaluate $\log \qu$ which is not always there}}

% If we parameterize $p(\xv|\zv, \uv)$ and $\pz$ (Lemmas~\ref{thm:reconstruction} and \ref{thm:elbo}) with $\theta \in \Theta$, then we can choose $\pxizu$ and $p_\theta(\zv)$ to be close to $\qxizu$ and $\qz$, respectively, by choosing $\theta$ that minimizes the expression $\pxizu$ and $p_\theta(\zv)$
In fact, we can choose %$\pxizu$ and $\pz$ (Lemmas~\ref{thm:reconstruction} and \ref{thm:elbo}) to be close to $\qxizu$ and $\qz$, respectively, by choosing 
$p(\xv|\zv, \uv)$ and $\pz$ that minimize
\s{missing theta}
$$
\KL(\qxizu \Vert \pxizu) + \KL(\qz \Vert p_\theta(\zv))
$$ 
While this expression seems difficult to compute, we introduce the following lemma that draws a connection to (conditional) variational autoencoders \citep{kingma2013auto} (VAEs):
\begin{lemma} \label{thm:vae}
For any valid distributions $\pz$ and $p(\xv | \zv, \uv)$
\begin{align*}
  & \bb{E}_{\qzu}\KL(\qxizu \Vert p(\xv|\zv, \uv)) + \KL(\qz \Vert \pz) \\
  = & \  \underbrace{\bb{E}_{\qxzu}[\KL(\qzixu \Vert \pz) - \log p(\xv | \zv, \uv)]}_{C_3: \text{Conditional VAE}} \\
  &  - \hq(\xv | \uv)
    \end{align*}
where $\hq(\xv|\uv)$ is the conditional entropy.
%$$
%\hq(\xv|\uv) = \sum_{\hat{\uv} \in \mc{U}} \hq(\xv|\uv = \hat{\uv}) \qu
%$$
\end{lemma}
% \s{use the underbrace to clearly indicate what is CVAE}
% \done{\rk{In the last line, I don't think there should be a negative in front of the KL term} \js{fixed}}
The final expression is the conditional VAE objective \citep{sohn2015learning,louizos2015the} plus the constant $-\hq(\xv | \uv)$ that does not depend on $\phi$, $p_\theta(\zv)$ or $\pxizu$.  If we parameterize $p(\xv|\zv, \uv)$ and $\pz$ with $\theta \in \Theta$, \s{missing theta} we can search for $\theta$ that minimizes the conditional VAE objective, which is tractable. Moreover, because $\hq(\xv | \uv)$ is constant wrt. both $\theta$ and $\phi$, optimizing the conditional VAE objective tightens the bounds.

% \s{you need to clearly say that 1) this is tractable and repeat that because H is a constant, this tightens the bounds}

% \s{this paragraph breaks the flow, consider moving to experiment section} 

% \done{\s{not sure i understand this paragraph}}

% \rk{Don't other people also use VAE to create good representations (not just as a generative model) aka. use $p$ to amortize $q_\phi$?} \js{that interpretation partly comes from shengjia (and is not super common), we should citep him}Our interpretation of the distributions $\pz$ and $p(\xv|\zv, \uv)$ is slightly different than the VAE interpretation: $\pz$ and $p(\xv|\zv, \uv)$ serve to amortize the aggregated posterior $\qz$ and posterior $\qxizu$ for the encoder $q_\phi$, as opposed to serving as the generative model; in other words, $p$ amortize $q_\phi$ and not vice versa. \todo[inline]{\js{maybe we should introduce amortization at some point}
% \s{i dont think we are amortizing..or do you mean the conditional piece?}
% \s{also, amortization usually hurts the bounds (but helps computationally). maybe that's something we should keep separate}}

% \s{next section is not readable/understandable. my suggestion. introduce the "VAE" bounds like current version. then discuss their limitation. then separate section on adversarial stuff}

% \s{We discuss the differences between $C_1$ and $C_2$ since they both provide a way to limit $\iq(\zv, \uv)$. 
% $C_1$ is guaranteed to be an upper bound to $\iq(\zv; \uv)$ but also upper-bounds $\iq(\xv; \zv | \uv)$ (which we would like to maximize), so it is more suitable when we value true guarantees on fairness over expressiveness. %\rk{Because p(z) is often chosen to be simple and the other p distributions are closer to q, }
% $C_2$ may more accurately approximate $\iq(\zv; \uv)$ but is guaranteed to be an upper bound only in the case of an optimal adversary; so it is more suitable when we are satisfied with guarantees on fairness in the limit of adversarial training, and we wish to learn more expressive representations.}

\subsection{A Tighter Bound to $\iq(\zv, \uv)$ via Adversarial Training}
% \s{here put the other upper bound lemma (the adversarial one), and move up minimax stuff from previous section here}

\s{i'm not sure we should call them loose vs. tight.}

\s{It would be tempting to use $C_1$, the tractable upper bound from Lemma~\ref{thm:elbo}, as a replacement for $\iq(\zv, \uv)$ in the constraint of eq. xxx. However, note from eq. yyy that $C_1$ is \emph{also} an upper bound to $\iq(\xv, \zv|\uv)$, which is the objective function (expressiveness) we would like to maximize in eq. 1.  If the constraint is too tight, we would constrain the expressiveness of our learned representations. Therefore, we introduce a tighter bound via the following lemma.}

The problem with using $C_1$, the upper bound in Lemma~\ref{thm:elbo} for the our only fairness constraint is that it is also an upper bound to $\iq(\xv, \zv|\uv)$. If the constraint is too tight, we would constrain the expressiveness of our learned representations. Therefore, we introduce a tighter bound via the following lemma.

\begin{lemma} \label{thm:adversarial}
For any distribution $\pu$
\begin{align}
\iq(\zv; \uv) = & \ \underbrace{\bb{E}_{\qz}\KL(\quiz \Vert \pu)}_{C_2: \text{Tight upper bound to }\iq(\zv; \uv)} - \KL(\qu \Vert \pu) \nonumber
\end{align}
%where 
%$$\quiz = \qzu / \qz$$
%and 
%$$\qz = \sum_{\xv, \uv} \qzixu \qxu$$
\end{lemma}

As $\uv$ is typically low-dimensional (e.g., a binary variable \s{cite xxx}), we can choose $\pu$ (Lemma~\ref{thm:adversarial}) to be a kernel density estimate based on the dataset $\mc{D}$. 
%In the particular case where $\uv$ is binary, we can choose $\pu$ to be a Bernoulli distribution with mean estimated from the dataset $\mc{D}_u$. 
By making $\KL(\qu \Vert \pu)$ as small as possible, our upper bound $C_2$ gets closer to $\iq(\zv, \uv)$.

While $\KL(\quiz \Vert \pu)$ is a valid upper bound to $\iq(\zv; \uv)$, according to Lemma~\ref{thm:adversarial}, $\quiz$ itself is not tractable, since again it requires at least integration over $\xv$. Our solution is to approximate $\quiz$ with a parametrized model $\puiz$ with parameters $\psi \in \Psi$:
\begin{equation}
 \argmin_\psi \bb{E}_{\qz}\KL(\quiz \Vert \puiz) % = \argmin_\psi - \bb{E}_{\qzu}[\log \puiz]
\end{equation}
which corresponds to maximum likelihood prediction with inputs $\zv$ and labels $\uv$ using $\puiz$. By replacing $\quiz$ with $\puiz$ in the tight upper bound ($\bb{E}_{\qz}\KL(\quiz \Vert \pu)$), we obtain a lower bound to that upper bound: 
% \rk{Is this equation correct? I can double check it if I have a sec...}\js{fixed}
\begin{align*}
    & \bb{E}_{\qzu}[\log \puiz - \log \pu] \\
    = & \ \bb{E}_{\qz}[\KL(\quiz \Vert \pu) - \KL(\quiz \Vert \puiz)] \\
    \leq & \ \bb{E}_{\qz}\KL(\quiz \Vert \pu)
\end{align*}
\s{all this math seems more complicated that it needs to be}
It follows that we can reduce $\iq(\zv; \uv)$ through the following adversarial training objective:
\begin{equation}
    \min_\phi \max_\psi \bb{E}_{\qzu}[\log \puiz - \log \pu]
\end{equation}
% where the minimization over $\phi$ occurs since we wish to reduce $\iq(\zv; \uv)$.
Here, the goal of the adversary is to minimize the difference between $\bb{E}_{\qzu}[\log \puiz - \log \pu]$ (the amortized ``upper bound'', which is tractable) and $\KL(\quiz \Vert \pu)$ (the true upper bound, which is not tractable). 

We summarize this in the following corollary:
\begin{corollary} \label{thm:adversarial-gap}
If $\KL(\quiz \Vert \puiz) \leq \ell$, then 
\begin{align}
    \iq(\zv; \uv) & \leq \bb{E}_{\qzu}[\log \puiz - \log \pu] \\
    & \quad - \KL(\qu \Vert \pu) + \ell \nonumber
\end{align}
for any distribution $p(\uv)$.
\end{corollary}
It immediately follows that when $\ell \to 0$, i.e. the adversary approaches global optimality, we obtain the true upper bound. 
% therefore, we can use the following computable constraint to achieve $\iq(\zv; \uv) < \epsilon$:
% \begin{equation}
% \bb{E}_{\qzu}[\log \puiz - \log \pu] < \epsilon  \label{eq:constraint-adversarial}
% \end{equation}
% \s{not sure i follow the therefore}

\subsection{A practical objective for controllable fair representations}
% \s{this section is hard to follow. need to add more test and remind the reader what you are trying to do..}
Recall that our goal is to find tractable estimates to the mutual information terms in Equation~\ref{eq:constraint-objective}, so that we can transform the objective into a more tractable one. In the previous sections, we have derived a lower bound for $\iq(\xv, \uv|\zv)$ (for which we want to maximize) and lower bounds for $\iq(\uv, \zv)$ (for which we want to minimize). Therefore, by applying Lemmas~\ref{thm:reconstruction}-\ref{thm:adversarial} to our objective from Equation~\ref{eq:constraint-objective}, we obtain the following practical objective, which involves constraints over the bounds over $\iq(\zv, \uv)$ and the conditional VAE objective: %\js{cite}:
% \rk{Does the $p_\psi$ below need to be changed?}
\begin{align}
 \min_{\theta, \phi} \max_{\psi \in \Psi} \quad  &  \mc{L}_r = - \bb{E}_{\qxzu}[\log \pxizu] \label{eq:tractable-objective} \\
\text{s.t.} \quad & C_1 = \bb{E}_{\qxu}\KL(\qzixu \Vert \pz) < \epsilon_1 \nonumber \\
    & C_2 = \bb{E}_{\qzu}[\log \puiz - \log \pu] < \epsilon_2  \nonumber \\
    % & \qquad \psi = \argmax_{\psi \in \Psi} \bb{E}_{\qzu}[\log \puiz] \nonumber \\
    & C_3 = \bb{E}_{\qxzu}[- \log \pxizu] \nonumber \\
    & \quad \quad + \KL(\qzixu \Vert \pz) < \epsilon_3 \nonumber
\end{align}
where $\mc{L}_r$, $C_1$, $C_2$ and $C_3$ are introduced in Lemmas~\ref{thm:reconstruction}, ~\ref{thm:elbo},~\ref{thm:adversarial} and~\ref{thm:vae} respectively.
\s{should $\psi$ also be an optimization variable next to theta and phi? the way this is written with the argmax is non-standard}\js{fixed}
\s{remind reader that these $c_i$ are defined in the lemmas}
\a{it might be helpful if we used the notations $\mc{L}_r$, $C_1$, $C_2$ etc. in previous subsections as well}
\js{I added them at the underbraces, do you think that works?}
\s{i think so, especially if you reference to them by name in the previous text}
% where we present the following interpretations and connections to existing quantities:

% $\mc{L}_r$ is the reconstruction loss and approximates $\iq(\xv; \zv | \uv)$ (Lemma~\ref{thm:reconstruction}), $C_1$ and $C_2$ approximate $\iq(\zv; \uv)$ (Lemmas~\ref{thm:elbo} and \ref{thm:adversarial}), and the constraint on $C_3$ encourages tightness of the approximations (Lemma~\ref{thm:vae}).

% The four lemmas introduces several bounds to the the mutual information terms in Equation~\ref{eq:constraint-objective}. In this subsection, we draw connections to existing components for learning fair representations.

% \xx{\paragraph{$\mc{L}_r$: Reconstruction Error} Minimizing the reconstruction error $- \bb{E}_{\qxzu}[\log \pxizu]$ encourages an autoencoding structure between $p_\theta$ and $q_\phi$. From Lemma~\ref{thm:reconstruction}, minimizing reconstruction error also maximizes a lower bound to $\iq(\xv; \zv | \uv)$, which is the primal objective of Equation~\ref{eq:constraint-objective}.

% \paragraph{$C_1$: Rate} The rate $\KL(\qzixu \Vert \pz)$ is an upper bound to $\iq(\zv; \uv)$, $\iq(\zv; \xv)$ and $\iq(\zv; \xv, \uv)$, according to Lemma~\ref{thm:elbo}. Therefore, the constraint over the rate immediately implies the following:
% \begin{equation}
%     \iq(\zv; \uv) < \epsilon; \qquad \iq(\zv; \xv) < \epsilon; \qquad \iq(\zv; \xv, \uv) < \epsilon
% \end{equation}
% which enforces a valid constraint over $\iq(\zv; \uv)$, while also limiting our ability to increase $\iq(\zv; \xv)$.}

% \paragraph{$C_3$: Adversarial Rate} 

% However, this does not lead to $\iq(\zv; \uv) < \epsilon$ since $\KL(\qu \Vert \pu) - \ell$ could be negative; if we are willing to assume the limit of adversarial training, i.e. $\ell$ is small, we can use the constraint in Equation~\ref{eq:constraint-adversarial}. Otherwise, we have the resort to the ``safer'' $C_1$ constraint and limit our potential to learn more informative $\zv$.

% \xx{\paragraph{$C_3$: Conditional VAE bound} 
% Constraining the conditional VAE bound encourages all bounds to be tight with respect to the true mutual information quantities, according to Lemma~\ref{thm:vae}.}

% \rk{This will be rewritten depending on the experiment results}
% As both $C_1 < \epsilon_1$ and $C_2 < \epsilon_2$ constrain $\iq(\zv; \uv)$... 
We discuss the differences between $C_1$ and $C_2$ since they both provide a way to limit $\iq(\zv, \uv)$. 
$C_1$ is guaranteed to be an upper bound to $\iq(\zv; \uv)$ but also upper-bounds $\iq(\xv; \zv | \uv)$ (which we would like to maximize), so it is more suitable when we value true guarantees on fairness over expressiveness. %\rk{Because p(z) is often chosen to be simple and the other p distributions are closer to q, }
$C_2$ may more accurately approximate $\iq(\zv; \uv)$ but is guaranteed to be an upper bound only in the case of an optimal adversary; so it is more suitable when we are satisfied with guarantees on fairness in the limit of adversarial training, and we wish to learn more expressive representations. \js{do we put it here, or right after adversarial section?}\s{either way works}

% We use $\qxu$ to denote the data distribution for $\mc{D}_u$, $\qzixu$ to denote the encoder distribution that is used to create a ``fair'' representation $\zv$ (parametrized by $\theta$).

% \s{does it make sense to have q deterministic vs stochastic?} \js{i think just stochastic would be fine? also we need the log-likelihood to compute one of the bounds}


% We wish to measure these mutual information under $\qxzu$, which can be factored into $\qzixu \qxu$.

% \s{justify conditioning on u}\js{added an explanation with the conditions}


% We can translate the conditional mutual information $\iq(\xv; \zv | \uv)$ into:
% \begin{align}
% \iq(\xv; \zv | \uv) & = \bb{E}_{\qxu}[\KL(\qzixu \Vert \pz)] - \KL(\qz \Vert \pz) \\
% & = \bb{E}_{\qxzu}[\log \pxizu] + H_q(\xv, u) + \KL(\qxuiz \Vert \pxuiz) 
% \end{align}

% \s{as a general rule, add intermediate derivations. we can comment out later, but it's good to have them in so we can double check for errors}

% which are tight when $\KL(\qxiz \Vert \pxiz)$ or $\KL(\qz) \Vert \pz)$ is small. In principle, $\pz$ can be arbitrarily chosen, but in the case of VAE it is usually fixed (and known as the ``prior'' of $\zv$). We can also choose $\pxzu$, which gives rise to the joint, which is $\pxzu = \pz \pxizu \qu$. 

% Both bounds are tight when $\KL(\qxzu \Vert \pxzu) = 0$, or equivalently $\KL(\qxziu \Vert \pxziu)) = 0$, because we can remove $\qu$ from both sides.

% Therefore, we can translate our objective to:
% \begin{gather} 
% \max \bb{E}_{\qxzu}[\log \pxizu] \\
% \text{s.t. } \iq(\zv; \uv) < \epsilon_1 \text{  and  } \KL(\qxziu \Vert \pxziu) < \epsilon_2
% \end{gather}
% which introduces another constraint to make sure that the bounds are tight. A feasible solution will satisfy 
% $$\iq(\xv; \zv | \uv) < \bb{E}_{\qxzu}[\log \pxizu] + \hq(\xv, \uv) + \epsilon_2$$

% \s{entropy piece is unknown. justify that this is OK}

% Turns out $\KL(\qxziu \Vert \pxziu)$ itself is exactly the VAE objective, so it is tractable through first-order Monte Carlo estimates, up to a constant:
% \begin{align*}
% &\ -\KL(\qxziu \Vert \pxziu)  \\
% & = \bb{E}_{\qxzu}[\log \pxizu] + \hq(\xv) - \bb{E}_{\qxu}\left[ \KL(\qzixu \Vert \pz) \right] \\
% & \equiv \bb{E}_{\qxzu}[\log p(\xv|\zv, u)]  - \bb{E}_{\qxu}\left[ \KL(\qzixu \Vert \pz) \right] 
% \end{align*}
% so we can base our constraints over the constant. \s{this could be tricky because we don't know the constant}

% \s{add the two versions separately, and discuss differences. including wrt existing work}


% For $\iq(\zv; \uv)$, we use an ``adversary'' to learn an encoding distribution $\puiz$ parametrized by $\psi$, such that $\puiz = \quiz$ is the optimal classifier of $\uv$ given $\zv$), and use the upper bound here:
% $$
% I_q(z; u) \leq \bb{E}_{\qz}[\KL(\quiz\Vert \pu)]
% $$
% which gives rise to our second constraint. $\pu$ can be obtained from fitting the empirical distribution of $\uv$. 

% This has the following intuition: our encoder wishes to ensure that it has low mutual information $\iq(z, u)$ under the distribution $\qzu$; we are able to sample from $\qzu$ and $\qu$ but not $\quiz$. The adversary serves to learn the conditional distribution $\quiz \propto \qzu / \qz$ through classification. The goal of our model is to prevent the adversary from doing this, through the upper bound, which selects $\qz$ such that $\quiz$ is close to $\qu$ .













% \subsection{Extensions to Equalized Odds and Equalized Opportunity}
% \rk{Can we move this to an appendix?}
% \rk{(Haven't edited this yet)}
% \js{wonder if this is crucial to our story; if not we may save some space}
% If we are also provided labels $y$ for a particular task, in the form of $\mc{D}_l = \{\xuyi\}_{i=1}^{M}$, we can also use the representations to predict $y$, which leads to a third condition:
% \begin{enumerate}
% \setcounter{enumi}{2}
%     \item $\zv$ can be used to classify $y$ with high accuracy. 
% \end{enumerate}
% We can either add this condition to the primal objective in Equation~\ref{eq:constraint-objective}, or add an additional constraint that we wish to have accuracy that is no less than a certain threshold. 

% With access to labels, we can also consider information-theoretic approaches to \textit{equalized odds} and \textit{equalized opportunity}. For \textit{equalized odds}, we require that $z$ and $u$ have low mutual information conditioned on the label, which is $I_q(\zv, \uv | \yv)$. For \textit{equalized opportunity}, we require that $z$ and $u$ have low mutual information conditioned on the label $y=1$, which is $I_q(\zv, \uv| y=1)$.

% We can still apply the upper bound almost as is:
% $$
% \iq(\zv; \uv) \leq \bb{E}_{\qzu}[\KL(\quizy \Vert \pu)]
% $$
% which can be implemented by using a separate classifier for each $y$ or using $y$ as input.
